Attention-Based Query Expansion Learning

Query expansion is a technique widely used in image search consisting in combining highly ranked images from an original query into an expanded query that is then reissued, generally leading to increased recall and precision. An important aspect of query expansion is choosing an appropriate way to combine the images into a new query. Interestingly, despite the undeniable empirical success of query expansion, ad-hoc methods with different caveats have dominated the landscape, and not a lot of research has been done on learning how to do query expansion. In this paper we propose a more principled framework to query expansion, where one trains, in a discriminative manner, a model that learns how images should be aggregated to form the expanded query. Within this framework, we propose a model that leverages a self-attention mechanism to effectively learn how to transfer information between the different images before aggregating them. Our approach obtains higher accuracy than existing approaches on standard benchmarks. More importantly, our approach is the only one that consistently shows high accuracy under different regimes, overcoming caveats of existing methods.

==> data.tex <==
\pgfplotstableread{
    nqe  avg  avgdecay  avgpdecay  aqe1  aqe2  aqe3 aqe4 aqe5  dqe  qel
    1  66.18  66.02  66.02  65.85  65.04  64.53  64.13  63.91  65.61  66.28
    2  67.26  66.71  66.86  66.75  65.83  65.02  64.52  64.18  67.19  67.08
    % 3  67.24  66.95  67.18  66.95  66.3  65.43  64.84  64.43  67.41  67.29
    4  66.9  67.34  67.48  67.53  66.8  65.83  65.03  64.59  67.68  67.78
    8  64.52  67.66  66.02  65.85  67.79  66.73  65.73  65.03  65.34  68.45
    12  64.99  66.99  64.92  64.99  67.79  67.26  66.12  65.32  65.28  68.8
    16  64.8  66.28  65.11  65.03  67.41  67.6  66.44  65.55  65.02  68.81
    20  64.66  65.69  65.02  65.06  66.53  67.86  66.68  65.69  64.97  68.97
    24  64.45  65.34  64.99  64.92  65.51  67.71  66.86  65.82  64.67  68.75
    28  64.34  65.24  64.97  64.84  65.23  67.69  66.99  65.92  64.63  68.89
    32  64.62  65.38  64.91  65.03  65.22  67.87  67.15  66.02  64.56  69.03
    36  64.29  65.46  64.93  65.16  65.27  68  67.23  66.09  64.52  68.95
    40  64.02  65.45  64.92  65.11  65.28  68.02  67.3  66.13  63.88  69.04
    44  63.79  65.43  64.86  64.98  65.21  68.04  67.34  66.16  63.51  69.28
    48  63.43  65.38  64.83  64.79  65.11  68  67.37  66.2  62.8  69.56
    52  63.42  65.39  64.78  64.73  65.08  68.01  67.43  66.23  62.66  69.69
    56  63.23  65.41  64.73  64.62  65.06  68.03  67.48  66.27  62.14  69.82
    60  62.37  65.39  64.62  64.4  64.98  68.02  67.51  66.3  62.04  69.78
    64  62.02  65.38  64.55  63.81  64.93  68.04  67.55  66.32  61.14  69.96
    68  61.61  65.36  64.46  63.69  64.94  68.08  67.6  66.36  61.32  70.02
    72  60.93  65.35  63.93  63.54  64.89  68.1   67.62  66.38  60.24  70.05
    76  60.17  65.33  63.77  63.37  64.85  68.09  67.64  66.4  60.6  70.06
    80  60.32  65.33  63.63  63.28  64.82  67.85  67.66  66.42  60.02  70.13
    84  59.53  65.34  63.49  63.18  64.81  67.82  67.67  66.43  59.52  70.08
    88  59.12  65.33  63.34  63.09  64.78  67.81  67.68  66.45  59.44  70.04
    92  58.47  65.32  63.19  62.99  64.72  67.82  67.69  66.46  59.48  70.01
    96  58.51  65.31  63.06  62.87  64.7  67.81  67.71  66.47  59.39  69.94
    100  57.62  65.27  62.94  62.72  64.68  67.8  67.72  66.48  58.41  69.86
    104  57.41  65.26  62.82  62.63  64.66  67.8  67.74  66.49  57.88  69.64
    108  57.21  65.25  62.65  62.5  64.57  67.79  67.74  66.49  58.41  69.51
    112  56.95  65.23  62.33  62.21  64.54  67.79  67.74  66.5  58.01  69.24
    116  56.82  65.22  62.19  62.12  64.53  67.78  67.74  66.5  57.92  69
    120  56.33  65.2  62.05  61.93  64.47  67.76  67.75  66.51  56.76  68.82
    124  55.88  65.17  61.9  61.78  64.44  67.75  67.76  66.52  57.25  68.61
    128  55.58  65.16  61.8  61.63  64.38  67.74  67.76  66.52  56.77  68.37
}{\nqetrends}
